Intermediate Defect Groups, Polarization Pairs, and Non-invertible Duality Defects

Within the framework of relative and absolute quantum field theories (QFTs), we present a general formalism for understanding polarizations of the intermediate defect group and constructing non-invertible duality defects in theories in $2k$ spacetime dimensions with self-dual gauge fields. We introduce the polarization pair, which fully specifies absolute QFTs as far as their $(k-1)$-form defect groups are concerned, including their $(k-1)$-form symmetries, global structures (including discrete $\theta$-angle), and local counterterms. Using the associated symmetry TFT, we show that the polarization pair is capable of succinctly describing topological manipulations, e.g., gauging $(k-1)$-form global symmetries and stacking counterterms, of absolute QFTs. Furthermore, automorphisms of the $(k-1)$-form charge lattice naturally act on polarization pairs via their action on the defect group; they can be viewed as dualities between absolute QFTs descending from the same relative QFT. Using this formalism, we present a prescription for building non-invertible symmetries of absolute QFTs. A large class of known examples, e.g., non-invertible defects in 4D $\mathcal{N}=4$ super-Yang--Mills, can be reformulated via this prescription. As another class of examples, we identify and investigate in detail a family of non-invertible duality defects in 6D superconformal field theories (SCFTs), including from the perspective of the symmetry TFT derived from Type IIB string theory.

==> tikz/ActionOnCharges.tex <==
\begin{tikzpicture}[scale= .4]

\node [style=none] (1) at (0,-5) {};
\node [style=none] (2) at (0,5) {};
\node [style=none] (3) at (4,10) {};
\node [style=none] (4) at (4,0) {};

\draw [style=black, fill=orange] (1.center) to (2.center) (2.center) to (3.center) (3.center) to (4.center) (4.center) to (1.center);


\end{tikzpicture}
